Efficient entity-based reinforcement learning

Recent deep reinforcement learning (DRL) successes rely on end-to-end learning from fixed-size observational inputs (e.g. image, state-variables). However, many challenging and interesting problems in decision making involve observations or intermediary representations which are best described as a set of entities: either the image-based approach would miss small but important details in the observations (e.g. ojects on a radar, vehicles on satellite images, etc.), the number of sensed objects is not fixed (e.g. robotic manipulation), or the problem simply cannot be represented in a meaningful way as an image (e.g. power grid control, or logistics). This type of structured representations is not directly compatible with current DRL architectures, however, there has been an increase in machine learning techniques directly targeting structured information, potentially addressing this issue. We propose to combine recent advances in set representations with slot attention and graph neural networks to process structured data, broadening the range of applications of DRL algorithms. This approach allows to address entity-based problems in an efficient and scalable way. We show that it can improve training time and robustness significantly, and demonstrate their potential to handle structured as well as purely visual domains, on multiple environments from the Atari Learning Environment and Simple Playgrounds.

==> figures/model.tex <==
\begin{figure}[ht]
	\centering
	\tikzstyle{block} = [rectangle, draw, text width=4em, text centered, rounded
	corners, minimum height=4em]

	\tikzstyle{line} = [draw, -latex]

	\begin{tikzpicture}[node distance = 0em, auto, thick]
		\node [block] (e) {Encoder};

		\node[xshift=8em, yshift=-3em, block] at (e) (p)  {Actor};
		\node[xshift=8em, yshift=3em, block] at (e) (v)  {Critic};

		\node[xshift=-3em] at (e.180) (o) {};
		\node[xshift=3em] at (p.0) (a) {};
		\node[xshift=3em] at (v.0) (vf) {};

		\path [line] (e.0) --++ (2em,0em) node [midway]{$l$} |-  (p.180);
		\path [line] (e.0) --++ (2em,0em) |- (v.180);
		\path [line] (o.0) -- node [midway]{$o$} (e.180);
		\path [line] (p.0) -- node [midway]{$a$} (a.0);
		\path [line] (v.0) -- node [midway]{$v_{f}$} (vf.0);
	\end{tikzpicture}
	\caption{Actor-critic model with shared latent vector $l$.}\label{fig:model}
\end{figure}


==> figures/rl.tex <==
\begin{figure}[ht]
	\centering
	\tikzstyle{block} = [rectangle, draw, text width=8em, text centered, rounded
	corners, minimum height=4em]

	\tikzstyle{line} = [draw, -latex]

	\begin{tikzpicture}[node distance = 6em, auto, thick]
		\node [block] (a) {Agent}; \node [block, below of=a] (e) {Environment};

		\path [line] (a.0) --++ (4em,0em) |- node [near start]{$a_t$} (e.0);
		\path [line] (e.190) --++ (-6em,0em) |- node [near start] {$o_{t+1}$} (a.170);
		\path [line] (e.170) --++ (-4.25em,0em) |- node [near start, right]	{$r_{t+1}$} (a.190);
	\end{tikzpicture}
	\caption{The RL agent's interaction with its environment}\label{fig:rl}
\end{figure}

